Sample size planning for pilot studies

Pilot studies are often the first step of experimental research. It is usually on a smaller scale and the results can inform intervention development, study feasibility and how the study implementation will play out, if such a larger main study is undertaken. This paper illustrates the relationship between pilot study sample size and the performance study design of main studies. We present two simple sample size calculation methods to ensure adequate study planning for main studies. We use numerical examples and simulations to demonstrate the use and performance of proposed methods. Practical heuristic guidelines are provided based on the results.

==> sections/intro.tex <==
Pilot studies are often conducted as the first step of experimental research. \citep{thabane2010, lancaster2004} It is usually on a smaller scale and the results can inform intervention development, study feasibility and how the study implementation will play out, if such a larger main study is undertaken. It also provides initial impression of treatment experience and the safety and efficacy profiles of treatments or interventions to help design the future main studies. \citep{thabane2010, lancaster2004, kistin2015} \citet{thabane2010} provides an extensive definition of a pilot study and what it entails, as well as a checklist for elements to be included in the pilot study. 

Different areas of research have recognized the importance of pilot studies and have published their findings, explaining what the results of the pilot study mean in the context of their field, such as critical care and reproductive health \citep{arnold2009, van2002}. Other authors \citep{thabane2010, lancaster2004} have addressed the importance and strength that pilot studies provide for a larger randomized controlled trial (RCT). RCTs in its entirety are extensive, time consuming, and costly, and have the potential to unexpectedly fail when thorough preparations are not done. If pilot studies are done prior, there is a certain degree of preparation which can provide a foundation for the subsequent confirmatory studies. \citet{lancaster2004} and \citet{arain2010} have reviewed both publications and published pilot studies in major medical journals from 2000-2001 and 2007-2008 to observe which pilot studies were deemed successful for the main trial, to provide guidelines for researchers conducting a pilot study. These papers have been successful in highlighting the ‘what’ and ‘why’ of pilot studies, however, there is still a lack of research and guidelines in designing pilot studies and determining an appropriate sample size for pilot studies.

Various recommendations for pilot sample size calculation have been proposed in response to the multipurpose nature of pilot studies.
\citet{hertzog2008} proposed to determine pilot study sample size based on estimates' precision and illustrated the relationship between pilot study sample size and constructed confidence intervals to meet various goals of pilot studies. 
\citet{cocks2013} recommended a confidence approach in pilot study to screen for intervention effects. \citet{julious2005} recommended a sample size of 12 per group for pilot studies based on feasibility, precision about the mean and variance, and regulatory considerations. \citet{viechtbauer2015} considered the sample size calculation of pilot studies with the goal of detecting potential problems aroused during the study. \citet{sim2012, whitehead2016, bell2018} advocated to estimate the pilot study sample size by minimizing the overall sample size needed for the pilot and the future study together. 

One important aspect in the research study design is to determine sample size such that there is sufficient power in demonstrating meaningful effects and achieving study goals. The estimates from the pilot study provide useful information in calculating the main study’s sample size.  A common approach is to use the observed effect size and outcome variability from the pilot study to perform sample size calculation for the main study. However, because pilot studies are inherently small, the estimates cannot be used with certainty. A small pilot study has a high potential to overestimate effect size or underestimate the variability, which may lead to an underpowered study design. Publications have suggested alternate methods to avoid this such as using confidence intervals, as well as addressing other issues, such as skewed data. \citet{browne1995, kieser1996, sim2012} recommended to use the upper confidence limit to reduce the chance of underestimating standard error in pilot studies when designing future studies. \citet{teare2014sample} used simulation to characterize the gain in precision in estimation and power of future studies as sample size increases in pilot study. \citet{westlund2017} highlighted the challenge and insufficiency to use pilot study data to determine whether to conduct or to design a confirmatory study.

In this paper, we presents alternative methods to calculate the sample size for the pilot study, such that the power calculation for the main study will be realistic with adequate performance. We illustrate the relationship between pilot study sample size and the power of the main study. We derive the pilot study sample size formula according to the desired quality of future study design, and use numerical examples to demonstrate the use of these methods.



==> sections/methods1b.tex <==
In this section we consider a one sample problem with a pilot study to quantify the study effect for the sample size planning of the main study. With the same setting in the previous section, we can consistently estimate $\mu$ with $ \bar{Y_p} = \ds \frac{\sum_{i=1}^{N_p} Y_i}{N_p}$ based on pilot samples. Assuming Normality and known variance $\sigma^2$, 
the sample mean $\bar{Y_p}$ follows a Normal distribution: 
\[
\bar{Y_p} \sim N( \mu, \frac{\sigma^2}{N_p})
\]

The hypothesis of interest for the main study is :
\[
H_0: \mu = 0 \quad \mbox{vs} \quad H_1: \mu > 0.
\]
Based on the sample mean $\bar{Y_p}$ from the pilot study, the sample size ($N_m^*$) required for the main study to have power of $1-\beta$ with type I error of $\alpha$ is
\[
N_m^*=(t_{1-\alpha/2} + t_{1-\beta})^2\frac{\sigma^2}{\bar{Y_p}^2},
\]
where $t_{1-\alpha/2}$ and $t_{1-\beta}$ are the upper ${\alpha/2}$ and ${\beta}$ percentiles of $t$-distribution. Comparing to the calculated sample size based on the true population mean $\mu$,
\[
N_m=(t_{1-\alpha/2} + t_{1-\beta})^2\frac{\sigma^2}{\mu^2},
\]
$N_m^*$ will provide an underpowered study design if $\bar{Y_p}$ overestimates the true mean $\mu$.

Therefore the pilot study design would require the pilot study sample size ($N_p$) to be large enough, such that the chance to overestimate $\bar{Y_p}$ is limited:
\[
N_p= \min\{N: \Pr(\bar{Y_p}) > \mu_L ) < p_0\},
\]
where $\mu_L$ and $p_0$ are pre-specified design parameters of lower bound threshold for the mean and tolerance probability. 

The distribution of sample mean $\bar{Y_p}$ is a function of sample size $N_p$. $\mu_U$ is related to the corresponding power ($1-\beta_L$) of the main study, through the calculated main study sample size $N_L$: 
\[
N_L=(t_{1-\alpha/2} + t_{1-\beta})^2\frac{\sigma^2}{\mu_L^2},
\],
and the corresponding power of the main study is
\[
1-\beta_L = 1- T_{\frac{\mu \sqrt{N_L}}{\sigma}}(t_{1-\alpha/2}).
\]
$T_\theta(\cdot)$ is the cumulative density function of non-central t-distribution with non centrality parameter $\theta$.

This calculation can also be useful when the goal is to quantify the effect size, which is the effect divided by standard deviation. The calculation using effect size with $sigma=1$ and the calculation based on actual effect with known $\sigma$ are mathematically identical.

 Algorithm 2 below presents the steps to calculate sample size for pilot studies for one sample problem with continuous outcomes. The goal is to limit the chance of both underpowered and overpowered study design for the main study, when using estimated study effect from the pilot study. 
 
\begin{enumerate}
\item Identify study and design parameters:
\begin{itemize}
    \item $\sigma$: known standard deviation of the outcome.  
    \item $\mu_0$:  study effect based on prior knowledge.
    \item $\alpha$ and $\beta$: the desired type I error and type II error of the main study
    \item $p_L$ and $\beta_L$: underpower probability and threshold; the main study is aimed to have less than $p_L$ chance with power lower than $1-\beta_L$.
    \item $p_U$ and $\beta_U$: overpower probability and threshold; the main study is aimed to have less than $p_U$ chance with power higher than power $1-\beta_U$.
\end{itemize}
\item Calculate the sample sizes of future studies corresponding the underpower and overpower thresholds:
\[
    N_L=(t_{1-\alpha/2} + t_{1-\beta_L})^2\frac{\sigma^2}{\mu_0^2},
\]
\[
    N_U=(t_{1-\alpha/2} + t_{1-\beta_U})^2\frac{\sigma^2}{\mu_0^2},
\]
\item Solve for corresponding values of study effect:
\[
    \mu_L=(t_{1-\alpha/2} + t_{1-\beta_L})\frac{\sigma}{\sqrt{N_L}},
\]
\[
    \mu_U=(t_{1-\alpha/2} + t_{1-\beta_U})^2\frac{\sigma}{\sqrt{N_U}},
\]
\item Calculate the pilot study sample size based underpower and overpower probability with the Normality assumption of sample mean:
\[
N_{pL}= \min\{N: \Pr(\bar{Y_p}(N) > \mu_L ) < p_L\} = \frac{z^2_{1-p_L}\sigma^2}{(\mu_L-\mu_0)^2}
\]
\[
N_{pU}= \min\{N: \Pr(\bar{Y_p}(N) < \mu_U ) < p_U\} =
\frac{z^2_{1-p_U}\sigma^2}{(\mu_0-\mu_U)^2}
\]
\item Calculate final sample size.
\[
N_p=\max\{ N_{pL}, N_{pU} \}
\]
\end{enumerate}

We can modify this algorithm for two sample comparison problem, where the main study compares the mean of two populations and its sample size calculation is based on the estimated difference between groups from the pilot data. We need to change Steps 2, 3, and 4 according to the sample size calculation formula for two sample comparison problem.



==> sections/methods2.tex <==
In this section we consider one sample pilot study design with binary outcomes. 
Let $Y_i$, with $\Pr(Y_i=1)=p$ and $\Pr(Y_i=0)=1-p$, be the binary outcome of interest for subject $i$, $i=1, \cdots, N_p$, where $N_p$ is the sample size of pilot study. The estimates generated from the pilot study can be used to facilitate the sample size calculation for the future confirmatory studies. 
Let $R= \sum Y_i$ represent the total number of responders. With the assumption that $Y_i$'s are iid, $R$ follows a binomial distribution with the parameters $N_p$ and $p$,
\begin{equation}
\label{eq1}
\Pr( R = r) = \left(
\begin{array}{c}
N_p\\
r
\end{array}
\right)
p^{r}(1-p)^{N_p-r}
\end{equation}
For the future study, the hypothesis of interest is:
\[
H_0: p = p_0 \quad \mbox{vs} \quad H_1: p > p_0
\]
There are many ways to perform the sample size calculation for binary data. Here we illustrate the calculation using the arcsin transformation technique. \citep{chow2003, cohen2013} The estimated response rate $\hat{p}=\ds \frac{r}{N_p}$ from the pilot study can be used to estimate $p$, and the effect size ($h_p$) and sample size ($N_f^*$) required for future studies with power of $1-\beta$ and type I error of $\alpha$ are
\begin{equation}
\label{eq2}
h_p = 2 \arcsin{\sqrt{\hat{p}}} - 2 \arcsin{\sqrt{p_0}} \\
N_{f}^*=\frac{(z_{1-\alpha/2} + z_{1-\beta})^2}{h_p^2},
\end{equation}
where $z_{1-\alpha/2}$ and $z_{1-\beta}$ are the upper ${\alpha/2}$ and ${\beta}$ percentiles of $z$-distribution. Comparing to the effect size and sample size needed based on the true response rate $p$,
\begin{equation}
\label{eq3}
h = 2 \arcsin{\sqrt{p}} - 2 \arcsin{\sqrt{p_0}} \\
N_f=\frac{(z_{1-\alpha/2} + z_{1-\beta})^2}{h^2},
\end{equation}
the sample size may be underestimated if $\hat{p}$ overestimates the true response rate $p$.

To ensure future study design has realistic power, we propose to calculate the sample size of pilot study such that there is a less than $q$ chance that the observed response rate $\hat{p}$ is greater than $p_U$
\begin{equation}
\label{eq4}
N_p= \min\{N: \Pr(\hat{p} > p_U ) < q \}
\end{equation}
where $p_U$ and $q$ are the design parameters of response rate threshold and confidence. $p_U$ then can be expressed in terms of the power ($1-\beta_U$) of future study through the calculated sample size ($N_U$) based on $p_U$;
\begin{equation}
\label{eq5}
h_U = 2 \arcsin{\sqrt{p_U}} - 2 \arcsin{\sqrt{p_0}} \\
N_U=\frac{(z_{1-\alpha/2} + z_{1-\beta})^2}{h_U^2},
\end{equation}
\begin{equation}
\label{eq6}
1-\beta_U = \Phi(h\sqrt{N_U}- z_{1-\alpha/2} )\\
\end{equation}
where $\Phi(\dot)$ is the cumulative density function of standard normal random variable.

More generally, one can limit the chance of both underpower and overpower for future study design. Algorithm 2 gives the steps to calculate sample size for one sample pilot studies with binary outcomes.
\begin{enumerate}
\item Identify study and design parameters:
\begin{itemize}
    \item $p$: true response rate of the outcome.
    \item $p_0$: clinically meaningful response rate of the outcome.
    \item $\alpha$ and $\beta$: the desired type I error and type II error for future studies.
    \item $q_L$ and $\beta_L$: confidence and threshold of underpower; the future confirmatory study will have less than $q_L$ chance to be underpowered with power of $1-\beta_L$.
    \item $q_U$ and $\beta_U$: confidence and threshold of overpower; the future confirmatory study will have less than $q_U$ chance to be overpowered with power of $1-\beta_U$.
\end{itemize}
\item calculate the sample sizes of future studies corresponding the underpower and overpower thresholds:
\[
    h = 2 \arcsin{\sqrt{p}} - 2 \arcsin{\sqrt{p_0}} \\
N_L=\frac{(z_{1-\alpha/2} + z_{1-\beta_L})^2}{h^2},
N_U=\frac{(z_{1-\alpha/2} + z_{1-\beta_U})^2}{h^2}.
\]
\item Solve for corresponding underpower and overpower thresholds:
\[
    h_L = \frac{z_{1-\alpha/2} + z_{1-\beta_L}}{\sqrt{N_L}}\\
    P_L= \sin^2(\frac{h_L}{2} + \arcsin{\sqrt{p_0}}) 
\]
\[
    h_U = \frac{z_{1-\alpha/2} + z_{1-\beta_U}}{\sqrt{N_U}}\\
    P_U= \sin^2(\frac{h_U}{2} + \arcsin{\sqrt{p_0}}) 
\]
\item calculate the pilot study sample size based on specified confidence :
\[
N_{pL}= \min\{N: \Pr(\hat{p} > p_L ) < q_L\}
\]
\[
N_{pU}= \min\{N: \Pr(\hat{p} < p_U ) < q_U\}
\]
\item Calculate final sample size.
\[
N_p=\max\{ N_{pL}, N{pU} \}
\]
\end{enumerate}
For easy implementation, step 3 can be approximated using arcsin square root transformation
\[
N_{pL}=\frac{z^2_{1-q_L}}{4(\arcsin{\sqrt{p_L}} - \arcsin{\sqrt{p}})^2}
\]
\[
N_{pU}=\frac{z^2_{q_U}}{4(\arcsin{\sqrt{p_U}} - \arcsin{\sqrt{p}})^2} 
\]

%% demonstrate using examples in the other papers




==> sections/methodsla.tex <==

In this section, we demonstrate our pilot sample size calculation method, when the outcome variability in the pilot study is incorporated in the sample size calculation of the main study.\citep{kistin2015}.  We first consider the one sample problem to compare the mean of a continuous variable to a pre-specified practically meaningful value.  Let $Y_i$ be the outcome of interest for subject $i$, $i=1, \cdots, N_p$, in the pilot study of sample size $N_p$.  Let $\mu$ and $\sigma^2$ be the population mean and variance of variable $Y$, pilot data sample mean ($\bar{Y}_p$)and variance ($S^2_p$) are consistent estimators for $\mu$ and $\sigma$, with $ \bar{Y_p} = \ds \frac{\sum_{i=1}^{N_p} Y_i}{N_p}$ and $S^2_p = \ds \frac{1}{N_p-1} \sum_{i=1}^{N_p} (Y_i-\bar{Y})^2$. With the Normality assumption, the sample variance $S^2_p$ follows a Chi-square distribution with $N_p-1$ degrees of freedom;
\[
\frac{(N_p-1) S^2_p}{\sigma^2} = \frac{\sum_{i=1}^{N_p} (Y_i-\bar{Y})^2}{ \sigma^2} \sim \chi^2_{N_p-1}
\]
and
\[
\Pr( S^2_p < \frac{\sigma^2}{N_p-1} \chi^2_{q, N_p-1}) = q
\]
where $\chi^2_{q, N_p-1}$ is the 100$q$th percentile of $\chi^2$ distribution with $N_p-1$ degrees of freedom.

The hypothesis of interest for the main study is:
\[
H_0: \mu = 0 \quad \mbox{vs} \quad H_1: \mu > 0,
\]
With a practically meaningful effect $\delta$ and the sample variance $S^2_p$ from the pilot study, the sample size ($N_m^*$) required for the main study to have power of $1-\beta$ with type I error of $\alpha$ is
\[
N_m^*=(t_{1-\alpha/2} + t_{1-\beta})^2\frac{S^2_p}{\delta^2},
\]
where $t_{1-\alpha/2}$ and $t_{1-\beta}$ are the upper ${\alpha/2}$ and ${\beta}$ percentiles of $t$-distribution. Comparing to the calculated sample size based on the true population variance $\sigma^2$,
\[
N_m=(t_{1-\alpha/2} + t_{1-\beta})^2\frac{\sigma^2}{\delta^2},
\]
$N_m^*$ will lead to an underpowered study design if $S^2_p$ underestimates the true variance $\sigma^2$. 

We propose to calculate the pilot study sample size such that the main study is more likely to have adequate power based on the pilot study estimate. This would require the pilot study sample size ($N_p$) to be large enough, such that the chance $S^2_p$ being severely underestimated is small:
\[
N_p= \min\{N: \Pr(S^2_p(N) < \sigma^2_L ) < p_0\},
\]
where $\sigma^2_L$ and $p_0$ are pre-specified design parameters of variance lower bound threshold and tolerance probability. 

The distribution of sample variance $S^2_p(N)$ is a function of sample size $N_p$. $\sigma^2_L$ is related to the corresponding power ($1-\beta_L$) of the main study, through the calculated main study sample size $N_L$: 
\[
N_L=(t_{1-\alpha/2} + t_{1-\beta})^2\frac{\sigma_L^2}{\delta^2},
\],
and the corresponding power of the main study is
\[
1-\beta_L = 1- T_{\frac{\delta \sqrt{N_L}}{\sigma}}(t_{1-\alpha/2}).
\]
$T_\theta(\cdot)$ is the cumulative density function of non-central t-distribution with non centrality parameter $\theta$.

More generally, we can consider the sample size calculation of pilot studies to limit the chance of both underpowered and overpowered study design for the main study. Algorithm 1 below presents the steps to calculate sample size for pilot studies for one sample problem with continuous outcomes.

\begin{enumerate}
\item Identify study and design parameters:
\begin{itemize}
    \item $\sigma$: standard deviation of the outcome based on prior knowledge.  
    \item $\delta$: practically important study effect.
    \item $\alpha$ and $\beta$: the desired type I error and type II error of the main study
    \item $p_L$ and $\beta_L$: underpower probability and threshold; the main study is aimed to have less than $p_L$ chance with power lower than $1-\beta_L$.
    \item $p_U$ and $\beta_U$: overpower probability and threshold; the main study is aimed to have less than $p_U$ chance with power higher than power $1-\beta_U$.
\end{itemize}
\item Calculate the sample sizes of future studies corresponding the underpower and overpower thresholds:
\[
    N_L=(t_{1-\alpha/2} + t_{1-\beta_L})^2\frac{\sigma^2}{\delta^2},
\]
\[
    N_U=(t_{1-\alpha/2} + t_{1-\beta_U})^2\frac{\sigma^2}{\delta^2},
\]
\item Solve for corresponding values of standard deviation:
\[
    \sigma^2_L=N_L \frac{\delta^2}{(t_{1-\alpha/2} + t_{1-\beta})^2},
\]
\[
    \sigma^2_U=N_U \frac{\delta^2}{(t_{1-\alpha/2} + t_{1-\beta})^2},
\]
\item Calculate the pilot study sample size based on the undepower and overpower probability with the $\chi^2$ distribution assumption of sample variance:
\[
N_{pL}= \min\{N: \Pr(S^2_p(N) < \sigma^2_L ) < p_L\}
\]
\[
N_{pU}= \min\{N: \Pr(S^2_p(N) > \sigma^2_U ) < p_U\}
\]
\item Calculate final sample size.
\[
N_p=\max\{ N_{pL}, N_{pU} \}
\]
\end{enumerate}
For easy implementation, step 3 calculation can be approximated\citep{canal2005} by
\[
N^*_{pL}=2*\frac{z^2_{1-p_L}}{(\frac{\sigma^2_L}{\sigma^2}-1)^2}+1
\]
\[
N^*_{pU}=2*\frac{z^2_{1-p_U})^2}{(\frac{\sigma^2_U}{\sigma^2}-1)^2}+1
\]
\[
N^*_p=\max\{ N^*_{pL}, N^*_{pU} \}
\]

where $z_{1-p_L}$ and $z_{1-p_U}$ are the upper ${p_L}$ and ${p_U}$ percentiles of $z$-distribution.

This method is easy to extend to two sample comparison situations, where the main study compares the mean of two populations and its sample size calculation is based on the (pooled) sample variance of the pilot data. We only need to change the sample size calculation formula from one sample to two sample comparison in steps 2 and 3.







==> sections/mynotes.tex <==

1.westlund 2017, 
use pilot study to determine where to conduct  a full trial 
